Lossy Compression for Lossless Prediction

Most data is automatically collected and only ever "seen" by algorithms. Yet, data compressors preserve perceptual fidelity rather than just the information needed by algorithms performing downstream tasks. In this paper, we characterize the bit-rate required to ensure high performance on all predictive tasks that are invariant under a set of transformations, such as data augmentations. Based on our theory, we design unsupervised objectives for training neural compressors. Using these objectives, we train a generic image compressor that achieves substantial rate savings (more than $1000\times$ on ImageNet) compared to JPEG on 8 datasets, without decreasing downstream classification performance.

==> appendices/checklist.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{In \cref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{In \cref{sec:conclusion} we mention the potential decrease in interpretability. }
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See \cref{appx:assumptions}.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See \cref{appx:proofs}. }
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code to train our main compressor is in \cref{appx:code_clip}, the code to replicate all our results is at \url{anonymous}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{The most important training details can be found at \cref{appx:reproducability}. Minor hyperparameters can be found in our code at  \url{anonymous}. }
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report error bars for MNIST (\cref{appx:mnist}) and Banana (\cref{appx:banana}). For larger experiments we sampled a fixed number of hyperparameters for each model and baseline (see \cref{appx:reproducability}), and report the best result.
    }
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{In \cref{appx:reproducability}.}
  \item Did you mention the license of the assets?
    \answerNo{} 
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Our clip compressor in \cref{appx:code_clip} and our code at \url{anonymous}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{We do not propose any new dataset. The main possible issues come from the CLIP dataset \cite{radford_learning_2021}, for which the data collection procedure is discussed in details in their paper.
    }
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
  \answerNo{We do not propose any new dataset.  The main possible issues come from the CLIP dataset \cite{radford_learning_2021}, for which the data collection procedure is discussed in details in their paper.
  }
\end{enumerate}

\end{enumerate}

==> figures/STL10/STL10_approx_invariance.tex <==
\begin{table}[h]
\caption{
Area under the rate-distortion curve (AURD).Distortion is VIC.
}
\begin{center}
\begin{tabular}{lr}
\toprule
Entropy models  & Lossless Rate & Lossless loss\\ 
\midrule 
0 	 	&1022.4	& 0.3075\\
0.05 	 	&3164.9 &0.3091	\\
0.2 	 	&694.5  &0.3324
0.5     	&2135.7 &0.3856
\bottomrule
\end{tabular}
\end{center}
\label{table:rate_variation_aurd}
\end{table}


\begin{figure}
    \centering
    \includegraphics{figures/STL10/rd_approx_invariance.pdf}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}


==> figures/STL10/STL10_distortions_old.tex <==
\begin{figure}[!htb]
    \centering
    \begin{minipage}{.44\textwidth}
        \centering
        \includegraphics[width=.9\textwidth]{figures/STL10/rd_dists_feat.pdf}
        \caption{Comparison of different distortions when the predictor is trained on the compressed representations.}
    \end{minipage}%
    \hspace{0.1\textwidth}
    \begin{minipage}{0.44\textwidth}
        \centering
        \includegraphics[width=.9\textwidth]{figures/STL10/rd_distsrec.pdf}
        \caption{Comparison of different distortions when the predictor is trained on reconstructions.}
    \end{minipage}
    \label{fig:rdistortions}
\end{figure}


==> figures/algorithms/BINCE_small.tex <==
\newcommand{\vspacing}{$\vphantom{\sum_{i}^t}$}
\begin{algorithm}[H]
%\caption{Single sample forward pass for BINCE}
\label{alg:BINCE_small}
    \begin{algorithmic}[1]
    \Require \vspacing $p_{\varphi}(\rv Z | \rv X)$,  ${\color{bluedark} q_{\theta}(\rv Z)}$, $f_{\psi}$, $\mathcal{D}$, $\rv A$, ${\color{bluedark} \beta}$, $n$ 
    \State \vspacing $m \leftarrow  \mathrm{select}(\mathcal{D})$  
    \State \vspacing $\tilde{x} \leftarrow A(m)$ \Comment{Augment}
    \State \vspacing $z \leftarrow \mathrm{sample}(p_{\varphi}(\rv Z | \tilde{x} ))$ 
    \State \vspacing ${\color{bluedark} \mathrm{rate\_loss}  \leftarrow - \log q_{\theta}(z)}$ 
    \State \vspacing $\{ m_i^- \}_{i=1}^n  \leftarrow  \mathrm{select}(\mathcal{D} \setminus \set{m})$ $n$ times  
    \State \vspacing $\tilde{\mathbf{x}} \leftarrow  [A(m), A(m_1^-), \dots, A(m_n^-)]$ 
    \State \vspacing $\mathbf{z}  \leftarrow \mathrm{sample}(p_{\varphi}(\rv Z | \mathbf{x}  ))$ 
    \State \vspacing $\mathrm{softmax} \leftarrow \frac{\exp f_{\psi}( z^{+}, z) }{(\sum_{z' \in \mathbf{z}} \exp f_{\psi}( z',  z))}$
    \State \vspacing $\mathrm{distortion\_loss}  \leftarrow - \log (\mathrm{softmax}) $  \\
    \Return \vspacing ${\color{bluedark} \mathrm{rate\_loss} + \beta} \cdot \mathrm{distortion\_loss}$
\end{algorithmic}
\end{algorithm}

==> figures/augmnist_plus/RD.tex <==
\begin{figure}[h]
     \centering
     \begin{subfigure}[h]{0.31\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/augmnist_plus/RD_curve_workshop_error.png}
         \caption{Rate-Error curve}
         \label{fig:augmnist++_RD}
     \end{subfigure}
     \begin{subfigure}[h]{0.68\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/augmnist_plus/rec_imgs_allin1_multirow.png}
         \caption{Reconstructions that allow $99\%$ downstream accuracy}
         \label{fig:augmnist++_RD_rec}
     \end{subfigure}
\caption{
By reconstructing prototypical digits, our VIC  achieves higher compression of augmented MNIST digits without hindering performance.
(a) The rate-error curve for MNIST classification, the area under the curve is $6.2 \pm 4.0$ for the invariant case and $12.0 \pm 10.0$ for the non invariant case.
%If instead you considered rate-log loss curves (as suggested by our theory) you would get 
(b) Reconstructions for the a non-invariant (second row) and invariant compressor (last row) that retains enough information for a downstream ResNet18 to classify the augmented MNISTs with $99\%$ test accuracy.
Our model only requires a a bit-rate of $48.1 \pm 0.5$ bits compared to $129.6 \pm 0.5 $ bits in the non invariant case.
All quantitative results are averaged over 5 runs.
}
\label{fig:augmnist++}
%\vspace{-0.5em}
\end{figure}

==> figures/augmnist_plus/RD_small.tex <==
\begin{figure}[h]
     \centering
     \begin{subfigure}[h]{0.3\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/augmnist_plus/RD_curve_workshop_error.png}
         \caption{Rate-Error curve}
         \label{fig:augmnist++_RD}
     \end{subfigure}
     \hfill{}
     \begin{subfigure}[h]{0.63\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/augmnist_plus/rec_imgs_allin1_multirow.png}
         \caption{Compression for $99\%$ accuracy}
         \label{fig:augmnist++_RD}
     \end{subfigure}
\caption{
Compression rates of augmented MNIST digits can be decreased  without hindering performance by reconstructing prototypical examples.
(a) Rate of a invariant (blue) and non-invariant (orange) neural compressors for various errors;
(b) Reconstructions of augmented digits (top) by a non-invariant (second row, $130$ bit-rate) and invariant compressor (last row, $48$ bit-rate) that retains enough information for reaching $99\%$ test accuracy.
}
\label{fig:augmnist++_experiment}
\vspace{-0.5em}
\end{figure}

==> figures/augmnist_plus/intro.tex <==
\begin{wrapfigure}{r}{0.41\textwidth}
\vspace{-\baselineskip}
\centering
\captionsetup[subfigure]{labelformat=empty}

\begin{subfigure}[h]{0.32\columnwidth}
 \centering
 \includegraphics[width=\textwidth]{figures/augmnist_plus/source.png}
 \caption{Source}
\end{subfigure}
\begin{subfigure}[h]{0.32\columnwidth}
 \centering
 \includegraphics[width=\textwidth]{figures/augmnist_plus/vae.png}
 \caption{Standard rec.}
\end{subfigure}
\begin{subfigure}[h]{0.32\columnwidth}
 \centering
 \includegraphics[width=\textwidth]{figures/augmnist_plus/ivae.png}
 \caption{Our rec.}
\end{subfigure}
  \vspace{-0.5em}
\addtocounter{figure}{-1} % for some reason adding 1 too much
 \captionof{figure}{
By reconstructing prototypical digits, our coder achieves higher compression without hindering performance.
(Left) source augmented MNIST digit; (center) a neural compressor optimized for perceptual similarity achieves a 130 bit-rate; (right)
our unsupervised invariant compressor achieves a 48 bit-rate.
 \label{fig:mnist_intro_large}
}


\end{wrapfigure}

==> figures/banana/RD_curves.tex <==
\begin{figure}[h]
 \centering
 \includegraphics[width=0.4\textwidth]{figures/banana/RD_curve_workshop.png}
\caption{
Rate-Distortion curve for a neural compressor and our invariant neural compressor, for compressing a banana distributed source for rotation invariant downstream tasks. 
We see that the invariant compressor significantly outperforms the non-invariant compressor, especially in low distortion regimes.
RD curves are generated by sweeping over $\beta$, the plotted curve is the average over 5 runs, standard errors for each $\beta$ are shown in gray (on the x and y axis).
}
\label{fig:bananas_RD_curves}
\vspace{-0.5em}
\end{figure}

==> figures/banana/intro.tex <==
\begin{wrapfigure}{r}{0.41\textwidth}
% \vspace{-\baselineskip}
\centering
\captionsetup[subfigure]{labelformat=empty}
\begin{subfigure}[h]{0.49\linewidth}
 \centering
 \includegraphics[width=\textwidth]{figures/banana/quantization_vae.png}
% \vspace*{-5mm}
%  \caption{Standard}
\end{subfigure}
%
\begin{subfigure}[h]{0.49\linewidth}
 \centering
 \includegraphics[width=\textwidth]{figures/banana/quantization_ivae_rot.png}
% \vspace*{-5mm}
%  \caption{Ours}
\end{subfigure}
  %\vspace{-1em}
  \addtocounter{figure}{-1} % for some reason adding 1 too much
 \captionof{figure}{
Compression rates of a Banana source \cite{balle_nonlinear_2020} can be decreased when downstream tasks are rotation invariant. (left) a neural transform coder achieves a 4.9 bit-rate; (right) our learned invariant transform coder achieves a 2.3 bit-rate.
Pink lines are quantization boundaries, dots are code vectors.
 \label{fig:banana_intro}
}
\vspace{-1.5\baselineskip}
\end{wrapfigure}


==> figures/banana/translation.tex <==
\begin{figure}[h]
     \centering
     \begin{subfigure}[h]{0.30\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/banana/quantization_vae.png}
         \caption{Standard Compression. }
         \label{fig:bananas_ytrnslt_vae}
     \end{subfigure}
     \hfill
     \begin{subfigure}[h]{0.30\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/banana/quantization_ivae_ytrnslt.png}
         \caption{$y$-translation Compression.}
         \label{fig:bananas_ytrnslt_ivae}
     \end{subfigure}
     \hfill
     \begin{subfigure}[h]{0.30\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/banana/quantization_ivae_xtrnslt.png}
         \caption{$x$-translation Compression.}
         \label{fig:bananas_xtrnslt_ivae}
     \end{subfigure}
\caption{
Similar to \cref{fig:banana_intro} for the case of downstream tasks that are invariant to translations. (left) standard compression achieves $4.86$
bit rate; (center) our compressor VIC compressor for $y$-translations achieves $3.24$ bit rate;
(center) our compressor VIC compressor for $x$-translations achieves a bit rate of $2.93$. 
All have a comparable similar invariant distortion.
}
\label{fig:bananas_trnslt}
\vspace{-0.5em}
\end{figure}

==> figures/intro_horizontal.tex <==
\begin{figure}[b]
\centering
\begin{minipage}{.54\textwidth}
\centering
 \includegraphics[width=0.99\linewidth]{figures/augmnist++/rec_imgs_allin1.png}
  \label{fig:mnist_intro}
  \vspace{-1em}
  \captionof{figure}{
Lossy compression of augmented MNIST digits (left) that allows $99\%$ downstream accuracy.
(center) A neural compressor optimized for perceptual similarity achieves a 130 bit-rate; (right)
our unsupervised invariant compressor achieves a 48 bit-rate.
}
\end{minipage}%
%
\hfill{}
%
\begin{minipage}{.43\textwidth}
\centering
 \includegraphics[width=0.49\linewidth]{figures/banana/quantization_vae.png}
 %\subcaption[]{}
 \includegraphics[width=0.49\linewidth]{figures/banana/quantization_ivae_rot.png}
  \label{fig:banana_intro}
  \vspace{-1em}
 \captionof{figure}{
Compression rates of a Banana source can be decreased when downstream tasks are rotation invariant. (left) a neural transform coder achieves a 5.4 bit-rate; (right) our learned invariant transform coder achieves a 2.5 bit-rate.
Pink lines are quantization boundaries, dots are code vectors.
}
\end{minipage}
\end{figure}

==> figures/intro_vertical.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-\baselineskip}
\centering
\captionsetup[subfigure]{labelformat=empty}
\begin{minipage}{.4\textwidth}
\centering
\begin{subfigure}[h]{0.49\linewidth}
 \centering
 \includegraphics[width=\textwidth]{figures/banana/quantization_vae.png}
% \vspace*{-5mm}
%  \caption{Standard}
\end{subfigure}
%
\begin{subfigure}[h]{0.49\linewidth}
 \centering
 \includegraphics[width=\textwidth]{figures/banana/quantization_ivae_rot.png}
% \vspace*{-5mm}
%  \caption{Ours}
\end{subfigure}
  %\vspace{-1em}
  \addtocounter{figure}{-1} % for some reason adding 1 too much
 \captionof{figure}{
Compression rates of a Banana source can be decreased when downstream tasks are rotation invariant. (left) a neural transform coder achieves a 5.4 bit-rate; (right) our learned invariant transform coder achieves a 2.5 bit-rate.
Pink lines are quantization boundaries, dots are code vectors.
 \label{fig:banana_intro}
}
\end{minipage}

\vspace{1em}

\begin{minipage}{.4\textwidth}
\centering
\begin{subfigure}[h]{0.32\columnwidth}
 \centering
 \includegraphics[width=\textwidth]{figures/augmnist++/source.png}
 \caption{Source}
\end{subfigure}\label{fig:mnist_intro}
\begin{subfigure}[h]{0.32\columnwidth}
 \centering
 \includegraphics[width=\textwidth]{figures/augmnist++/vae.png}
 \caption{Standard rec.}
\end{subfigure}
\begin{subfigure}[h]{0.32\columnwidth}
 \centering
 \includegraphics[width=\textwidth]{figures/augmnist++/ivae.png}
 \caption{Our rec.}
\end{subfigure}
  \vspace{-1em}
    \addtocounter{figure}{-1} % for some reason adding 1 too much
 \captionof{figure}{
Our coder achieves better compression by only keeping the information that is necessary for desired tasks.
(Left) source augmented MNIST digit; (center) a neural compressor optimized for perceptual similarity achieves a 130 bit-rate; (right)
our unsupervised invariant compressor achieves a 48 bit-rate.
 \label{fig:mnist_intro}
}
\end{minipage}%
%
\vspace{-1.5\baselineskip}
\end{wrapfigure}

==> figures/objectives/bince.tex <==
%\input{figures/algorithms/BINCE_small}


\begin{figure}[h]
\centering
\begin{subfigure}{0.51\linewidth}
\includegraphics[width=\linewidth]{figures/objectives/objectives-BINCE_neurips_minimal.pdf}
%\caption{BINCE for image compression}
%\caption{DIB with neural networks}
%\label{fig:dib_neural_net}
\end{subfigure}
%
\hfill
%
\makebox[0.45\linewidth][l]{\begin{subfigure}{0.45\linewidth}
\small
%\SetInd{0.3em}{0.6em}
\input{figures/algorithms/BINCE_small}
\vspace{-1em}
%\caption{Algorithm for BINCE's forward pass}
%\label{alg:pseudo_dib}
\end{subfigure}}
%
\caption{
BINCE in practice. The only difference with contrastive SSL (InfoNCE) is the \textcolor{bluedark}{entropy bottleneck}.
(Left) Illustration of BINCE in the case of images compression and invariance to data augmentations.
(Right) Algorithm for BINCE's forward pass (not batched).
}\label{fig:BINCE}
\end{figure}


==> figures/objectives/ivae.tex <==

\begin{figure}
\centering
\begin{subfigure}{0.53\linewidth}
\small
\begin{algorithmic}[1]
    %\Require Encoder $p_{\varphi}(\rv Z | \rv X)$,  Entropy Model $q_{\theta}(\rv Z)$,  Decoder $q_{\phi}(\rv X | \rv Z)$
    \Require Dataset $\mathcal{D}$,  Random augmenter $\rv A$, $\beta$
    \State $m  \leftarrow  \mathrm{select}(\mathcal{D})$  \Comment{Sample}
    \State $\tilde{x} \leftarrow A(m)$ \Comment{Augment}
    \State $z \leftarrow \mathrm{sample}(p_{\varphi}(\rv Z | \tilde{x} ))$ \Comment{Encode}
    \State $\mathrm{rate\_loss} \leftarrow - \log q_{\theta}(z) $ \Comment{Entropy Bottleneck}
    \State $\mathrm{distortion\_loss}  \leftarrow - \log q_{\phi}(x | z) $ \Comment{Direct Distortion} \\
    Return $\mathrm{rate\_loss} + \beta \cdot \mathrm{distortion\_loss}$
\end{algorithmic}
\caption{Training Algorithm}
 \label{fig:vic_algorithm}
\end{subfigure}
%
\begin{subfigure}{0.37\linewidth}
\includegraphics[width=\linewidth]{figures/objectives/objectives-ivae_neurips_cycle.pdf}
\caption{Model}
 \label{fig:vic_model}
\end{subfigure}
\caption{
...}
\end{figure}


==> figures/objectives/objectives_old.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.37\linewidth}
\includegraphics[width=\linewidth]{figures/objectives/objectives-ivae_neurips_minimal.pdf}
\vspace*{-2em}
\caption{VIC}
\label{fig:VIC}
\end{subfigure}
%
\hfill
%
\begin{subfigure}{0.47\linewidth}
\includegraphics[width=\linewidth]{figures/objectives/objectives-BINCE_neurips_minimal.pdf}
\vspace*{-2em}
\caption{BINCE}
\label{fig:BINCE}
\end{subfigure}
%
\caption{
Our unsupervised objectives for image compression and invariance to data augmentation.
(a) VIC is a standard neural compressor where inputs are \textcolor{burntorange}{augmented} but not target reconstructions.
(b) BINCE ensures that compressed representations can still be used to discriminate which inputs are augmented version of one another. 
It is a constrastive SSL model with an \textcolor{bluedark}{entropy bottleneck}.
}\label{fig:objectives}
\end{figure}


==> figures/objectives/vic.tex <==
\begin{wrapfigure}{r}{0.41\textwidth}
\vspace{-\baselineskip}
 \centering
 \includegraphics[width=\linewidth]{figures/objectives/objectives-ivae_neurips_minimal.pdf}
\caption{
THe only 
}
\vspace{-1.5\baselineskip}
\end{wrapfigure}

==> tables/clip_linear.tex <==
\begin{table}[h]
\caption{
\tofill{}
}
\scriptsize
\center
\begin{tabular}{llrrrrrrrrr}
\toprule
 &  & ImageNet  & STL & PCam & Cars & CIFAR10 & CIFAR100 & Food      & Pets & Caltech  \\ % 
\midrule 
\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering ~Bit-Rate   }} 
& CLIP & 1.52e4  & 1.52e4 & 1.52e4 & 1.52e4 & 1.52e4  & 1.52e4  & 1.52e4     & 1.52e4 & 1.52e4  \\ 
 & CLIP+EB\textsuperscript{$-$} & ImageNet  & 2.46e3 & PCam & 2.60e3 & 2.53e3 & CIFAR100 & Food      & 2.32e3 & 2.46e3  \\ 
  & CLIP+EB & ImageNet  & 1.34e3 & PCam & 1.47e3 & 1.41e3 & 1.41e3 & Food      & 1.21e3 & 1.34e3  \\
 & CLIP+EB\textsuperscript{$+$}  & ImageNet  & 9.52e2 & PCam & 1.07e3 & 1.02e3 & CIFAR100 & Food      & 8.35e2 & 9.53e2  \\ 
  \midrule 
\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering ~Test Acc.   }} 
 & CLIP  \cite{radford_learning_2021} & 76.1  & 98.3 & 83.9 & 81.8 & 95.1 & 80.5 & 88.8      & 90.0 & 93.0  \\ 
 & CLIP+EB\textsuperscript{$-$} & ImageNet  & 98.7 & PCam & 80.8 & 95.0 & CIFAR100 & Food      & 89.1 & 93.7  \\ 
 & CLIP+EB & ImageNet  & 98.7 & PCam & 80.0 & 94.8 & 79.0 & Food    & 88.3 & 93.7  \\ 
 & CLIP+EB\textsuperscript{$+$}  & ImageNet  & 98.6 & PCam & 78.9 & 94.4 & CIFAR100 & Food      & 87.8 & 93.5  \\ 
\bottomrule
\end{tabular}
\label{table:clip_all}
\end{table}

==> tables/clip_linear_text.tex <==
\begin{table}[h]
\caption{
\tofill{}
}
\footnotesize{}
\center
\begin{tabular}{llrrrrrrrr}
\toprule
 &  & ImageNet  & STL & PCam & Cars & CIFAR10  & Food      & Pets & Caltech  \\ % 
\midrule 
\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering ~Rate [Bits]   }} 
& CLIP & 1.52e4  & 1.52e4 & 1.52e4 & 1.52e4 & 1.52e4    & 1.52e4     & 1.52e4 & 1.52e4  \\ 
  & CLIP+EB & ImageNet  & STL & PCam & Cars & CIFAR10 & Food      & Pets & Caltech  \\ 
 & CLIP+EB$^-$ & ImageNet  & STL & PCam & Cars & CIFAR10  & Food      & Pets & Caltech  \\ 
 & CLIP+EB$^+$  & ImageNet  & STL & PCam & Cars & CIFAR10  & Food      & Pets & Caltech  \\ 
  \midrule 
\multirow{4}{*}{\rotatebox[origin=c]{90}{\centering ~Test Acc. [\%] }} 
& CLIP \cite{radford_learning_2021} &  76.1  & 98.3  &  83.9 & 81.8 &  95.1   & 88.8      &  90.0 & 93.0  \\ 
 & CLIP+EB & ImageNet  & STL & PCam & Cars & CIFAR10 & Food    & Pets & Caltech  \\ 
  & CLIP+EB$^-$ & ImageNet  & STL & PCam & Cars & CIFAR10  & Food      & Pets & Caltech  \\ 
 & CLIP+EB$^+$  & ImageNet  & STL & PCam & Cars & CIFAR10 & Food      & Pets & Caltech  \\ 
\bottomrule
\end{tabular}
\label{table:clip_linear_text}
\end{table}

==> tables/clip_no_EB.tex <==
\begin{table}[h]
\vspace{-1\baselineskip}
\caption{
Using our entropy bottleneck (EB) on CLIP compresses representations without decreasing test predictions.
$\Delta$ denotes the difference between CLIP and our CLIP+EB.
}
\small
\center
\begin{tabular}{lrrrrrrrrr}
\toprule
& ImageNet  & STL & PCam & Cars & CIFAR10 & Food     & Flowers  & Pets  \\ % Food101  / cars / PCAM / Galaxy zoo 2 / text / SUN397 / DTD / oxford pets /caltech 101 / flowers 102 / mnist
% different tasks on galaxy
\midrule 
% JPEG Bit-Rate & 1.39e6  & 2.1e5  & 9.2e4 & 8.1e5 &  2.40e4 & 3.4e5 \\
% Lossyless Bit-Rate & 1350   & 1050 &  1450 & 1350 & 1350 &1350  \\
Rates CLIP+EB [Kb] &  \tofill{}  & \tofill{} &  \tofill{}  & \tofill{} &\tofill{} & \tofill{} & \tofill{} & \tofill{}  \\ % cifar 100 & $14\times$
Rates CLIP [Kb]  &   \tofill{} &  \tofill{} &   \tofill{}  & \tofill{} &  \tofill{} &  \tofill{} & \tofill{} & \tofill{}  \\ % cifar 100 & $14\times$
\midrule 
$\Delta$ gen. gap $[\%]$  & \tofill{}    & \tofill{}  & \tofill{}  &  \tofill{}  &  \tofill{} &   \tofill{}  & \tofill{} & \tofill{}  \\
$\Delta$ test acc. $[\%]$ &   \tofill{}   &   \tofill{}  &  \tofill{}  &   \tofill{}  &  \tofill{} &  \tofill{}  & \tofill{} & \tofill{}  \\
\bottomrule
\end{tabular}
\label{table:clip_no_EB}
\end{table}

==> tables/max_invariant.tex <==
\begin{table}[ht!]
\centering
\caption{Examples of maximal invariants $M(\cdot)$.
}
\label{table:max_inv}
\begin{tabular}{@{}lr@{}}
\toprule
Equivalence relation
& $M(x)$\\ \midrule
$x_2$-Translation $\vec x + [0,t]^T$ & $x_1$ \\
Scaling $c \cdot \vec x$ & $\vec x / x_n$ \\
Rotations & Norm:  $\| \vec x \|_2$ \\
Function $f(\vec x)$  & $f(\vec x)$ \\
Permutations & Empirical measure \\
Graphs Isomorphisms & canonization \\
$\sim_1$ and $\sim_2$  & $M_1(M_2(\vec x))$ \\
 \bottomrule
\end{tabular}
\end{table}
